Efficient Greedy Discrete Subtrajectory Clustering

We cluster a set of trajectories T using subtrajectories of T. Clustering quality may be measured by the number of clusters, the number of vertices of T that are absent from the clustering, and by the Fr\'{e}chet distance between subtrajectories in a cluster. A $\Delta$-cluster of T is a cluster ${\mathcal{P}}$ of subtrajectories of T with a centre $P \in {\mathcal{P}}$ with complexity $\ell$, where all subtrajectories in ${\mathcal{P}}$ have Fr\'{e}chet distance at most $\Delta$ to $P$. Buchin, Buchin, Gudmundsson, L\"{o}ffler and Luo present two $O(n^2 + n m \ell)$-time algorithms: SC($\max$, $\ell$, $\Delta$, T) computes a single $\Delta$-cluster where $P$ has at least $\ell$ vertices and maximises the cardinality $m$ of ${\mathcal{P}}$. SC($m$, $\max$, $\Delta$, T) computes a single $\Delta$-cluster where ${\mathcal{P}}$ has cardinality $m$ and maximises the complexity $\ell$ of $P$. We use such maximum-cardinality clusters in a greedy clustering algorithm. We provide an efficient implementation of SC($\max$, $\ell$, $\Delta$, T) and SC($m$, $\max$, $\Delta$, T) that significantly outperforms previous implementations. We use these functions as a subroutine in a greedy clustering algorithm, which performs well when compared to existing subtrajectory clustering algorithms on real-world data. Finally, we observe that, for fixed $\Delta$ and T, these two functions always output a point on the Pareto front of some bivariate function $\theta(\ell, m)$. We design a new algorithm PSC($\Delta$, T) that in $O( n^2 \log^4 n)$ time computes a $2$-approximation of this Pareto front. This yields a broader set of candidate clusters, with comparable quality. We show that using PSC($\Delta$, T) as a subroutine improves the clustering quality and performance even further.

==> plots/real_centers.tex <==

    \begin{figure} \begin{center}

        \begin{tikzpicture}[scale=0.8]
            \begin{axis}[
                title={},
                xlabel={Number of points},
                ylabel={Time in seconds},
                legend pos=north west,
                scaled ticks=false,
                width={0.4\textwidth},
            ]

            \addplot+[only marks] coordinates { (1792084, 75281.8) (896335, 36240.3) (598054, 22433.4) (448468, 15839.2) (358926, 11912.6) (299688, 9426.77)};
            \addlegendentry{Drop points};

            \addplot+[only marks] coordinates { (1792084, 75281.8) (899784, 15287.2) (585907, 6131.19) (450666, 3428.07) (367449, 2223.06) (291571, 1369.46)};
            \addlegendentry{Drop trajectories};


            \end{axis}
        \end{tikzpicture}%


        \caption{Running time of \textbf{kCentre} on the Difter data set with $c_1 = 1, c_2 = 200, c_3 = 2011$.
        We have no algorithms to directly compare our performance to, but we can illustrate that we terminate correctly and in good time. The running time appears to scale quadratically, which is to be expected from an $O(|C| \cdot z \log^4 n) \subset O(|C| \cdot n^2 \log^4 n)$-time algorithm. 
        When the input has almost two million vertices, our algorithm uses 10 GB of memory and approximately 20 hours of running time. 
        }
        \label{fig:drifter}

    \end{center} \end{figure}


==> plots/real_table.tex <==

    \begin{figure*} \begin{center}
    \begin{tabular}{@{}lrrcrrrrrr@{}}
        \toprule
        Name & Seconds & GBytes & Clusters & Max Frechet & Avg Frechet & kMeans & kCenters & Max Size & Avg Size\\
        \midrule
        kMeans-length & 4.59 & 0.01 & 24 & 1506.66 & 229.13 & 54.62 & 509.89 & 22 & 6.29\\
kMeans-size & 3.10 & 0.03 & 34 & 1150.38 & 223.27 & 30.62 & 386.91 & 6 & 3.56\\
\textbf{kMeans} & 5.75 & 0.01 & 28 & 894.71 & 153.18 & 27.04 & 301.55 & 32 & 7.14\\
AFMNPT & 112.32 & 0.13 & 16 & 1340.97 & 307.22 & 23.88 & 423.02 & 27 & 8.50\\
BBGHSSSSSW & 22.87 & 3.75 & 261 & 501.25 & 134.79 & 219.02 & 420.88 & 41 & 8.17\\
kCenter-length & 1.97 & 0.01 & 15 & 204.77 & 164.99 & 52.76 & 115.01 & 34 & 10.00\\
kCenter-size & 3.03 & 0.01 & 21 & 102.38 & 81.69 & 87.23 & 118.06 & 108 & 21.19\\
\textbf{kCenters} & 2.97 & 0.01 & 35 & 102.36 & 62.52 & 65.32 & 95.32 & 78 & 28.74\\
        \bottomrule
    \end{tabular}

        \caption{Various statistics on the clusterings obtained from different algorithms on athens small. kMeans algorithms and scores use $c_1 = 0.5, c_2 = 0.0003, c_3 = 128$. kCenters algorithms and scores use $c_1 = 1, c_2 = 0.3, c_3 = 128$.
        The -length algorithms use $l = 15$. The -size algorithms use $s = 6$.}

    \end{center} \end{figure*}


==> plots/real_table_chicago.tex <==

    \begin{figure} \begin{center}
    \begin{tabular}{@{}lrrcrrrrrr@{}}
        \toprule
        Name & Seconds & GBytes & Clusters & Max Frechet & Avg Frechet & kMeans & kCenters & Max Size & Avg Size\\
        \midrule
        kMeans-length & 1946.54 & 0.05 & 88 & 1346.11 & 38.08 & 179.97 & 1552.41 & 65 & 18.58\\
kMeans-size & 1084.04 & 0.69 & 108 & 666.00 & 83.04 & 86.89 & 797.58 & 6 & 4.46\\
kMeans-this & 280.39 & 0.03 & 75 & 829.85 & 61.75 & 56.92 & 910.42 & 42 & 10.97\\
agarwal & 10634.65 & 3.98 & 39 & 1661.83 & 142.49 & 49.26 & 1702.77 & 40 & 17.54\\
java & 2732.21 & 9.21 & 957 & 156.53 & 27.25 & 619.26 & 1133.62 & 74 & 15.82\\
kCenter-length & 296.50 & 0.08 & 55 & 84.97 & 73.25 & 178.24 & 259.84 & 91 & 26.55\\
kCenter-size & 361.39 & 0.06 & 48 & 169.95 & 112.12 & 813.27 & 232.20 & 1816 & 481.04\\
kCenters-this & 137.70 & 0.03 & 74 & 42.48 & 31.69 & 80.85 & 151.40 & 65 & 13.69\\
        \bottomrule
    \end{tabular}

        \caption{Various statistics on the clusterings obtained from different algorithms on Chicago with $1/4$ trajectories. kMeans algorithms and scores use $c_1 = 0.5, c_2 = 0.0003, c_3 = 888$. kCenters algorithms and scores use $c_1 = 1.0, c_2 = 1.0, c_3 = 888$.
        The -length algorithms use $l = 15$. The -size algorithms use $s = 6$.}

    \end{center} \end{figure}


==> plots/real_table_scaled.tex <==

    \begin{figure*} \begin{center}
    \begin{tabular}{@{}lrrcrrrrrr@{}}
        \toprule
        Name & Seconds & GBytes & Clusters & Max Frechet & Avg Frechet & kMeans & kCenters & Max Size & Avg Size\\
        \midrule
        kMeans-length & 185.20 & 0.09 & 22 & 818.60 & 139.52 & 53.89 & 304.99 & 22 & 6.95\\
kMeans-size & 54.47 & 0.18 & 31 & 1289.21 & 186.60 & 29.01 & 426.57 & 6 & 3.71\\
\textbf{kMeans} & \textbf{29.08} & \textbf{0.02} & \textbf{30} & \textbf{665.08} & \textbf{108.67} & \textbf{24.93} & \textbf{234.93} & \textbf{17} & \textbf{5.63}\\
AFMNPT & 1304.49 & 0.87 & 17 & 2054.68 & 234.55 & 24.56 & 637.43 & 28 & 11.00\\
BBGHSSSSSW & 270.25 & 2.98 & 969 & 441.73 & 44.15 & 565.64 & 1109.70 & 52 & 6.28\\
kCenter-length & 54.22 & 0.10 & 16 & 102.39 & 87.45 & 58.04 & 93.32 & 33 & 9.19\\
kCenter-size & 52.98 & 0.03 & 26 & 204.80 & 117.88 & 343.21 & 104.16 & 1250 & 341.96\\
\textbf{kCenters} & \textbf{18.51} & \textbf{0.01} & \textbf{24} & \textbf{102.33} & \textbf{81.80} & \textbf{32.78} & \textbf{70.11} & \textbf{65} & \textbf{10.12}\\
        \bottomrule
    \end{tabular}

        \caption{Various statistics on the clusterings obtained from different algorithms on athens small with $4 \times$ subdivision. kMeans algorithms and scores use $c_1 = 0.5, c_2 = 0.0003, c_3 = 128$. kCenters algorithms and scores use $c_1 = 1, c_2 = 0.3, c_3 = 128$.
        The -length algorithms use $l = 60$. The -size algorithms use $s = 6$.}

    \end{center} \end{figure*}

